Analysis of Two-Stage Rollout Designs with Clustering for Causal Inference under Network Interference

Estimating causal effects under interference is pertinent to many real-world settings. Recent work with low-order potential outcomes models uses a rollout design to obtain unbiased estimators that require no interference network information. However, the required extrapolation can lead to prohibitively high variance. To address this, we propose a two-stage experiment that selects a sub-population in the first stage and restricts treatment rollout to this sub-population in the second stage. We explore the role of clustering in the first stage by analyzing the bias and variance of a polynomial interpolation-style estimator under this experimental design. Bias increases with the number of edges cut in the clustering of the interference network, but variance depends on qualities of the clustering that relate to homophily and covariate balance. There is a tension between clustering objectives that minimize the number of cut edges versus those that maximize covariate balance across clusters. Through simulations, we explore a bias-variance trade-off and compare the performance of the estimator under different clustering strategies.

==> 4-clustering.tex <==
\mccomment{Do we need a transition sentence?}
\section{Using Clusters to Choose \texorpdfstring{$\cU$}{U}} 
\label{sec:cluster_results}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/two_stage.png}
    \caption{An illustration of a two-stage rollout design. In the first stage, we select a subset of the clusters as the experimental group $\cU$. In the second stage, we carry out a rollout design on the units in $\cU$ and deterministically assign the remaining units to control.}
    \label{fig:two_stage}
\end{figure}

In Theorem \ref{thm:bias}, \mcedit{we see that the estimator is not unbiased in general. It turns out that bias comes from edges crossing between $\cU$ and $[n]\setminus\cU$. We see that the bias depends on $\Pr(\cS\subseteq\cU)$, the probability that a subset of an individual's in-neighborhood is selected in the first stage of the design.} A natural question to consider is if a clever choice of $\cU$ reduces this bias. 

To formalize this, we adopt the following notation. A clustering $\Pi$ of the interference network is a partition of $[n]$; $\pi \in \Pi$ is a subset $\pi \subseteq [n]$ of units assigned to the same cluster. Given a unit $i \in [n]$, we define $\pi(i)$ as the cluster containing $i$. Given $\cS\!\subseteq\![n]$, we define $\Pi(\cS) := \{ \pi \in \Pi \ | \ \exists \; i\!\in\!\cS \colon \pi = \pi(i) \}$. 

\mcedit{Suppose the population is grouped in $n_c$ clusters, each of size $n/n_c$, and in the first stage of the design entire clusters are selected into $\cU$ according to a completely randomized design $\emph{CRD}(\tfrac{p}{q}n_c,n_c)$. For ease of presentation, assume fractions evaluate to integers. Then, the probability that a given subset $\cS$ is in $\cU$ is given by $\big[\tfrac{(p/q)n_c}{n_c}\big]_{|\Pi(\cS)|}$.}

\begin{corollary} \label{coro:bias}
    Under a $\beta$-order potential outcomes model, a clustering $\Pi$ of $n_c$ equal-size clusters, and a \mcedit{$\emph{CRD}(\beta,k,\ncU)$ Two-Stage Rollout Design where units in the first stage are selected if their cluster is selected and clusters are selected according to $\emph{CRD}(\tfrac{p}{q}n_c,n_c)$, the bias is given by}
    \[
       \tfrac{1}{n} \sum_{i=1}^n \sum_{\cS \in \cS_i^\beta \setminus \varnothing} c_{i,\cS} \Big[\tfrac{q}{p}\big[\tfrac{(p/q)n_c}{n_c}\big]_{|\Pi(\cS)|} - 1\Big]
    \]
\end{corollary}
\mcedit{If for all $i\in[n], \cS\subseteq\cN_i$ we have $|\Pi(\cS)|=1$, then $\big[\tfrac{(p/q)n_c}{n_c}\big]_{|\Pi(\cS)|}=\tfrac{p}{q}$ and the estimator is unbiased. This latter condition holds when $\beta=1$, since this would restrict $|\cS|=1$ and thus $\Pi(S)=1$. Alternatively, when the clustering $\Pi$ of the network is such that there are no cut edges, that is the graph contains no edges with endpoints from two distinct clusters, then any in-neighborhood must be entirely contained in a single cluster and the condition holds.}
\mcedit{One benefit of the two-stage estimator introduced in Section~\ref{sec:newmethod} is that it does not require structural knowledge of the underlying interference network. However, since cut edges contribute to bias, utilizing a clustering of the network that minimizes the number of edges crossing clusters will also minimize the bias of the estimator. This would require information about the network.} 

\mccomment{Hmm not entirely what else to say here. Previously this transitioned to some experimental results, but I'm not sure that's in the right place anymore.}

\subsection{Variance under Two-Stage Design with Clustering}
To provide some theoretical insight into how the extrapolation and sampling variances depend on $q$, we present variance bounds using the clustering framework.
Let $Y_{\max}$ be a bound on the potential outcomes.

\begin{theorem} \label{thm:var_bounds_clustering}
    For any $\beta$, under a {$\emph{Bern}(\beta,\Pi,p,q)$} Two-Stage Rollout Design, we may bound:
    {
    \begin{align*}
         \E_{\cU}\Big[\underset{\bz}{\emph{Var}}\big(\widehat{\emph{TTE}}\big)\Big] &\leq 
        \tfrac{1}{q^{2(\beta-1)}} \cdot \tfrac{Y_{\max}^2d^2\beta^{2\beta}(\beta+1)^2}{np^2} \\
        \underset{\cU}{\emph{Var}} \Big( \E_{\bz} \big[ \widehat{\emph{TTE}} \big] \Big) &\leq 
        \mcdelete{q \cdot \underset{\pi \in \Pi}{\max} \,|\pi| \cdot \tfrac{Y_{\max}^2d^2}{np}},
    \end{align*}}
\end{theorem}

\mccomment{Variance of conditional expectation should be $\tfrac{qY_{\max}^2d^2}{pnn_c}$?}

{In each of these bounds, the last fraction depends on the parameters of the network and the potential outcomes ($n, Y_{\max}, d, \beta$) as well as the treatment budget $p$, whereas the earlier factors depend on parameters of the two-stage experimental design ($q$ and $\Pi$). These bounds align with our observations from Figure~\ref{fig:visualize_tradeoff}; namely, the extrapolation variance is a decreasing function and the sampling variance an increasing function of $q$. Importantly, we see that the extrapolation variance is constant with respect to $q$ when $\beta\!=\!1$, while the sampling variance grows linearly in $q$. This agrees with the behavior we see in Figure~\ref{fig:compare_amazon_clusterings}. When $\beta\geq2$, the extrapolation variance decreases significantly with $q$, reducing the total variance at the cost of incurring some sampling variance. This suggests that the estimator performs better under the two-stage design than the one-stage design when $\beta>1$.} Below, we will show that the scaling with $q$ in these bounds is tight for $\beta \in \{1,2\}$. Finally, the $1/n$ scaling in both bounds tells us that as the size of the network increases, the variance will tend to $0$ as long as the potential outcomes remain bounded and the network degree scales as $d = o(\sqrt{n})$.

\subsection{Explicit variance formula when \texorpdfstring{$\beta=1$}{beta=1}}

Recall that our parameterization of the potential outcomes in \ref{eq:ppom} is in terms of the \textit{incoming} effects to agent $i$, $c_{i,\cS}$. However, it will often be useful in our calculations to flip perspectives and reason about the \textit{outgoing} effects (or \textit{influences}). To this end, for $\cS \subseteq [n]$, let us define
\[
L_\cS := \sum_{i : \cS\subseteq\cN_i} c_{i,\cS}
\]
When $\cS=\{j\}$ for some $j\in[n]$, we write $L_j$ to align with the definition of \citet{yu2022PNAS}. Following their convention, $L_j$ is the influence of treating an individual $j$ on their and their neighbors' outcomes. We interpret $L_\cS$ as the contribution to the $\TTE$ of jointly treating all individuals in $\cS$. The following theorem gives an exact expression for the variance when $\beta=1$ in terms of these $L_j$ effects.
\mcedit{
\begin{theorem} \label{thm:variance-deg1-crd} 
Under a potential outcomes model with $\beta=1$, the polynomial interpolation estimator under a Two-Stage Rollout Design with clustering has variance
\[
    \tfrac{1-q}{pn - q} \widehat{\Var_{j\in[n]}}(L_j) \ + \ \tfrac{(p-q)(1-pn)}{p(pn-q)(n_c-1)} \widehat{\Var_{\pi\in\Pi}}\Big(\widehat{\E}_{j\in\pi}[L_j]\Big)
\]
\end{theorem}
}

\mcedit{The proof is in Appendix \ref{app:clusters}. When $q=1$, the design is a simple cluster randomized design where every selected cluster in the first stage is treated in the second stage, and the variance expression simplifies to $\tfrac{1-p}{p(n_c-1)} \widehat{\Var}_{\pi\in\Pi}\big(\widehat{\E}_{j\in\pi}[L_j]\big)$. This aligns exactly with the cluster-randomized result from \citet{yu2022PNAS}.
When $q=p$, our variance expression is $\tfrac{1-p}{p(n-1)} \widehat{\Var}_{j\in[n]}(L_j)$ and aligns exactly with the completely randomized design result from \citet{yu2022PNAS}.}
\mccomment{Add some more explanation here as to why they match?}

\mccomment{Everything from this point forward still needs to be updated as of 10/7/24.}

\mcdelete{
\begin{theorem} \label{thm:variance-deg1} 
Under a potential outcomes model with $\beta=1$, the polynomial interpolation estimator under $\textrm{Bern}(\Pi,p,\mathbf{q})$ Two-Stage Rollout Design has variance
\[
    \emph{Var}\Big[ \widehat{\emph{TTE}}_{\emph{PI}} \Big] = \tfrac{1}{n^2p} \sum_{\pi \in \Pi} \bigg[ (1-q) \sum_{j \in \pi} L_j^2 \ + \ (q-p) \Big( \sum_{j \in \pi} L_j \Big)^2 \bigg].
\]
\end{theorem}
}

The following result gives us a practical recommendation for choosing $q$.
% \mcedit{
% \begin{corollary}
%     \label{coro:deg1-variance-empirical-moments}
%     The variance in Theorem \ref{thm:variance-deg1} can we rewritten as
%     \[
%     \emph{Var}\Big[ \widehat{\emph{TTE}}_{\emph{PI}} \Big] = \tfrac{1}{n^2p} \sum_{\pi \in \Pi} \Big( |\pi|(1-q) + |\pi|^2(q-p) \Big) \E_{j \in \pi} \big[ L_j^2 \big] 
%     - \tfrac{q-p}{n^2p} \sum_{\pi \in \Pi} |\pi|^2 \Var_{j \in \pi} \big( L_j \big)
%     \]
%     where $\E\limits_{j \in [n]}$ denotes an empirical average and $\underset{j \in \pi}{\emph{Var}} $ denotes an empirical variance.
% \end{corollary}
% }
% \begin{proof}
%     Picking up from Equation \eqref{eq:lawofTV-deg1-simple}, we have \meedit{
% \begin{align*}
%    \eqref{eq:lawofTV-deg1-simple} &= \tfrac{1}{n^2p} \sum_{\pi \in \Pi} \bigg[ \Big(1-q + |\pi|(q-p) - |\pi|(q-p)\Big) \sum_{j \in \pi} L_j^2 + (q-p) \Big( \sum_{j \in \pi} L_j \Big)^2 \bigg] \\
%     &= \tfrac{1}{n^2p} \sum_{\pi \in \Pi} \bigg[ \Big(1-q + |\pi|(q-p)\Big) \sum_{j \in \pi} L_j^2 \bigg] 
%     - \tfrac{q-p}{n^2p} \sum_{\pi \in \Pi} \bigg[ |\pi| \sum_{j \in \pi} L_j^2 - \Big( \sum_{j \in \pi} L_j \Big)^2 \bigg] \\
%     &= \tfrac{1}{n^2p} \sum_{\pi \in \Pi} \bigg[ \Big(1-q + |\pi|(q-p)\Big) \sum_{j \in \pi} L_j^2 \bigg] 
%     - \tfrac{q-p}{n^2p} \sum_{\pi \in \Pi} |\pi|^2 \bigg[ \E_{j \in \pi} \big[ L_j^2 \big] - \Big( \E_{j \in \pi} \big[ L_j \big] \Big)^2 \bigg] \\
%     &= \tfrac{1}{n^2p} \sum_{\pi \in \Pi} \bigg[ \Big(1-q + |\pi|(q-p)\Big) \sum_{j \in \pi} L_j^2 \bigg] 
%     - \tfrac{q-p}{n^2p} \sum_{\pi \in \Pi} |\pi|^2 \Var_{j \in \pi} \big( L_j \big) \\
%     &= \tfrac{1}{n^2p} \sum_{\pi \in \Pi} \Big( |\pi|(1-q) + |\pi|^2(q-p) \Big) \E_{j \in \pi} \big[ L_j^2 \big] 
%     - \tfrac{q-p}{n^2p} \sum_{\pi \in \Pi} |\pi|^2 \Var_{j \in \pi} \big( L_j \big) \\
% \end{align*} 
% }
% \end{proof}


\begin{corollary} \label{coro:deg1 q=p}
    When $\beta=1$ and the influence terms $L_j$ have the same sign for all $j\in[n]$, then the variance of the two-stage estimator under a $\textrm{Bern}(\Pi,p,q)$ Two-Stage Rollout Design is minimized when $q=p$.
\end{corollary}

In other words, this corollary tells us that we should not cluster the network to correlate the treatment assignments when $\beta=1$; rather, we are better off using the polynomial interpolation estimator with a $\textrm{Bern}(\beta,p)$ Rollout design. Experiments in Section \ref{sec:experiments} give us intuition for Corollary \ref{coro:deg1 q=p}. In particular, we see that for $\beta=1$, the extrapolation variance is relatively small. Thus, incurring \textit{any} sampling variance from the two-stage design is too costly. As is evident in the proof, the same-signs assumption is sufficient but not necessary for this optimality result.



==> 6-conclusion.tex <==
\section{Conclusion}
While it is possible to get unbiased estimates of the total treatment effect without using any knowledge of the underlying interference network using polynomial interpolation and a Bernoulli staggered rollout design, the required polynomial extrapolation results in very high variance under a $\beta$-order potential outcomes model with $\beta > 1$. We propose a two-stage experiment design where in the first stage we employ a clustering of the interference network to select a subset of the population. In the second stage, we utilize a Bernoulli staggered rollout to assign treatment to those selected by the first stage. This greatly reduces the variance due to extrapolation when $\beta>1$, but at the cost of incurring bias and sampling variance. Via numerical simulations on stochastic block models as well as three real-world network datasets, we explore the tradeoff between error due to extrapolation and error due to sampling. It is clear that when $\beta>1$, the proposed design decreases the error of the polynomial interpolation estimator such that it outperforms baseline estimators. However, when $\beta=1$, we recommend the simple Bernoulli rollout design since the proposed two-stage design increases the overall error of the estimator. Our theoretical results, including an explicit expression for the bias and a bound on the variance of the estimator, validate our empirical findings. We also empirically explore the impact of the clustering on the performance of the estimator. We find, somewhat surprisingly, that even utilizing a random clustering of the network (which uses no knowledge of its structure) in the proposed two-stage design greatly reduces the overall error of the polynomial interpolation estimator. This tells us that in settings where $\beta>1$, the variance due to extrapolation is the dominating portion of the error, such that reducing it is critical to reducing the error overall. 

A limiting aspect of our results is that we require correct specification of the potential outcomes model. Incorrect specification of the model could lead to drawing incorrect causal conclusions, which could have negative impacts in domains where a decision-maker relies on these results. This plagues many works, not just our own. A critical direction for future work is analyzing the effects of model misspecification. An important related direction is model selection, particularly designing or proposing methods for determining the model parameter $\beta$, as it is most likely unknown a priori, but required for correct model specification. Perhaps the most limiting assumption in our work is that the network and potential outcomes do no vary with time. Since this is not likely to hold in many settings, especially on online platforms, we are interested in exploring avenues for handling time-dependence in future work. Finally, due to the polynomial interpolation, we only use $\beta+1$ points for a $\beta$-order model. Ongoing work includes analyzing the value of additional measurements. 

==> a4-misspecification.tex <==
\section{Connection to Model Misspecification when \texorpdfstring{$q=1$}{q=1}}
\label{app:misspecification}

The 1-Stage estimator from \citet{cortez2022neurips} is 
\begin{equation} \label{eq:estimatorDefn-1Stage}
    \widehat{\TTE}_{\textrm{1-Stage}}^{\beta} := 
        \frac{1}{n} \sum\limits_{i=1}^{n}  \sum\limits_{t=0}^{\beta} \Big( \ell_{t,p}(1) - \ell_{t,p}(0) \Big) \cdot Y_i(\mathbf{z}^t),
        \quad
        \ell_{t,p}(x) = \prod_{\substack{s=0 \\ s\not=t}}^{\beta} \tfrac{\beta x-ps}{pt-ps}.
\end{equation}

\mccomment{Need to go back and make it explicit that the model parameter $\beta$ may be different from the estimator parameter $\beta$. Maybe the model one should be $\beta^*$? Or maybe we just pick a completely different letter for the estimator?}

When evaluating the estimator with $\beta=1$, the estimator is simply
\begin{equation} \label{eq:beta=1 estimator}
    \widehat{\TTE}_{\textrm{1-Stage}}^{\beta=1} = \frac{1}{np} \sum\limits_{i=1}^{n} \Big( Y_i(\bz^1) - Y_i(\bz^0) \Big)
\end{equation}

\subsection{Equivalence of the degree 1 estimator to other estimators}
\begin{theorem}
    Under a {$\emph{Bern}(\beta=1,p,q)$} Two-Stage Rollout Design, the 2-stage estimator defined in \eqref{eq:estimatorDefn} is equivalent to the estimator defined in equation \eqref{eq:beta=1 estimator}.
\end{theorem}

\begin{proof}
    Under a {$\emph{Bern}(\beta,p,q)$} Two-Stage Rollout Design with $\beta=1$, we have that 
    \[
    \ell_{t,q}(1) - \ell_{t,q}(0) = \prod_{\substack{s=0 \\ s\not=t}}^{1} \tfrac{1-qs}{qt-qs} \ - \ \prod_{\substack{s=0 \\ s\not=t}}^{1} \tfrac{-qs}{qt-qs}.
    \]
    When $t=0$, we have
    \[
    \ell_{0,q}(1) - \ell_{0,q}(0) = \frac{1-q}{-q} \ - \ \frac{-q}{-q} = -\frac{1}{q},
    \]
    and when $t=1$, we have
    \[
    \ell_{1,q}(1) - \ell_{1,q}(0) = \frac{1}{q} \ - \ 0.
    \]
    Plugging this into the estimator defintion in \eqref{eq:estimatorDefn} for $\beta=1$, we have 
    \begin{align*}
        \widehat{\TTE}_{\textrm{2-Stage}} &= \frac{q}{np} \sum_{i=1}^n \Big(Y_i(\bz^0)\big(\ell_{0,q}(1) - \ell_{0,q}(0)\big) \ + \ Y_i(\bz^1)\big(\ell_{1,q}(1) - \ell_{1,q}(0)\big) \Big) \\
        &= \frac{q}{np} \sum_{i=1}^n \Big(Y_i(\bz^1)\cdot\frac{1}{q} \ - \ Y_i(\bz^0)\cdot\frac{1}{q}\Big) \\
        &= \frac{1}{np} \sum\limits_{i=1}^{n} \Big( Y_i(\bz^1) - Y_i(\bz^0) \Big)\\
        &= \widehat{\TTE}_{\textrm{1-Stage}}^{\beta=1}
    \end{align*}
\end{proof}

\begin{theorem} \label{thm:q=1,2-stage,equivalence}
    Under a {$\emph{Bern}(\beta,p,q=1)$} Two-Stage Rollout Design, the 2-stage estimator defined in equation \eqref{eq:estimatorDefn} is equivalent to the estimator defined in \eqref{eq:beta=1 estimator}.
\end{theorem}
\begin{proof}
    Under a {$\emph{Bern}(\beta,p,q)$} Two-Stage Rollout Design with $q=1$, we have 
    \[
    \ell_{t,q}(1) - \ell_{t,q}(0) = \prod_{\substack{s=0 \\ s\not=t}}^{\beta} \tfrac{\beta-s}{t-s} \ - \ \prod_{\substack{s=0 \\ s\not=t}}^{\beta} \tfrac{-s}{t-s}.
    \]
Notice that when $t\in\{1,2,\ldots,\beta-1\}$, i.e. $t\ne0$ and $t\ne\beta$, at some point we have a term corresponding to $s=0$ and $s=\beta$ in the products above. Thus, both products evaluate to $0$.

When $t=0$, we have 
\[
\ell_{t,q}(1) - \ell_{t,q}(0) \ = \ \prod_{\substack{s=1}}^{\beta} \tfrac{\beta-s}{0-s} \ - \ \prod_{\substack{s=1}}^{\beta} \tfrac{-s}{0-s} \ = \ \prod_{\substack{s=1}}^{\beta} \tfrac{\beta-s}{-s} \ - \ 1 \ = \ -1
\]
because the product equals $0$ due to the $s=\beta$ term. Similarly, when $t=\beta$, we have 
\[
\ell_{t,q}(1) - \ell_{t,q}(0) \ = \ \prod_{\substack{s=0}}^{\beta-1} \tfrac{\beta-s}{\beta-s} \ - \ \prod_{\substack{s=0}}^{\beta-1} \tfrac{-s}{\beta-s} \ = \ 1
\]
since the second product will equal $0$ due to the $s=0$ term.
To summarize, we have
\[
\ell_{t,q}(1) - \ell_{t,q}(0) = 
\begin{cases}
    -1 & t = 0\\
    0 & 1 \leq t \leq \beta-1 \\
    1 & t = \beta
\end{cases}.
\]
\end{proof}

\subsection{Results}
Note that per Theorem \ref{thm:bias}, when $q=1$, and stage 1 is unit Bernoulli, we have
    \[
        \E \Big[ \widehat{\TTE}_{\emph{2-Stage}} \Big] - \TTE = \tfrac{1}{n} \sum_{i=1}^n \sum_{\cS \in \cS_i^\beta \setminus \varnothing} c_{i,\cS} \Big[ p^{|\cS|-1} - 1 \Big].
    \]

\begin{theorem}
    Suppose there exists $\beta^*>1$ such that for all $i\in[n]$ we have $Y_i(\bz):= \sum_{\cS\subseteq \cS_i^{\beta^*}}c_{i,\cS}\prod_{j\in\cS}z_j$. Then, under a {$\emph{Bern}(\beta=\beta^*,p,q=1)$} Two-Stage Rollout Design, or a {$\emph{Bern}(\beta=1,p)$} One-Stage Rollout Design, the estimator defined in equation \eqref{eq:beta=1 estimator} has bias 
    \[
        \E \Big[  \widehat{\TTE}_{\textrm{1-Stage}}^{\beta=1} \Big] - \TTE = \tfrac{1}{n} \sum_{i=1}^n \sum_{\cS \in \cS_i^{\beta^*} \setminus \varnothing} c_{i,\cS} \Big[ p^{|\cS|-1} - 1 \Big].
    \]
\end{theorem}

\begin{proof}
    This follows from Theorems \ref{thm:bias} and \ref{thm:q=1,2-stage,equivalence}.
\end{proof}

\begin{theorem}
    Suppose there exists $\beta^*>1$ such that for all $i\in[n]$ we have $Y_i(\bz):= \sum_{\cS\subseteq \cS_i^{\beta^*}}c_{i,\cS}\prod_{j\in\cS}z_j$. Then, under a {$\emph{Bern}(\beta=\beta^*,p,q=1)$} Two-Stage Rollout Design, or a {$\emph{Bern}(\beta=1,p)$} One-Stage Rollout Design, the estimator defined in equation \eqref{eq:beta=1 estimator} has variance
    \[
        \Var \Big[  \widehat{\TTE}_{\textrm{1-Stage}}^{\beta=1} \Big] \leq \frac{d^2Y_{\max}^2}{np}.
    \]
\end{theorem}
\begin{proof}
Where $z_j$ is the treatment assigment of individual $j$ in the final stage of the staggered rollout (either $T=1$ or $T=\beta^*$ depending on the design), we have
    \begin{align*}
        \Var \Big[  \widehat{\TTE}_{\textrm{1-Stage}}^{\beta=1} \Big] &= \Var \bigg[ \frac{1}{np} \sum_{i\in[n]} \sum_{\substack{\cS \in \cS_i^{\beta^*} \\ \cS\ne0}} c_{i,
        \cS} \prod_{j\in\cS} z_j  \bigg] \\
        &= \frac{1}{n^2p^2} \sum_{i\in[n]} \sum_{i'\in[n]} \sum_{\substack{\cS \in \cS_i^{\beta^*} \\ \cS\ne0}} c_{i,\cS} \sum_{\substack{\cS' \in \cS_{i'}^{\prime\beta^*} \\ \cS'\ne0}} c_{i',
        \cS'} \ \Cov\Big(\prod_{j\in\cS} z_j, \ \prod_{j'\in\cS'} z_{j'}\Big) \\
        &= \frac{1}{n^2p^2} \sum_{i\in[n]} \sum_{i'\in\cM_i} \sum_{\substack{\cS \in \cS_i^{\beta^*} \\ \cS\ne0}} c_{i,\cS} \sum_{\substack{\cS' \in \cS_{i'}^{\prime\beta^*} \\ \cS'\ne0}} c_{i',
        \cS'} \ \Big(p^{|\cS\cup\cS'|} - p^{|\cS|+|\cS'|}\Big) \\
        &\leq \frac{1}{n^2p^2} \sum_{i\in[n]} \sum_{i'\in\cM_i} \sum_{\substack{\cS \in \cS_i^{\beta^*} \\ \cS\ne0}} c_{i,\cS} \sum_{\substack{\cS' \in \cS_{i'}^{\prime\beta^*} \\ \cS'\ne0}} c_{i',
        \cS'} \ p^{|\cS\cup\cS'|} \\
        &\leq \frac{1}{n^2p} \sum_{i\in[n]} \sum_{i'\in\cM_i} \sum_{\substack{\cS \in \cS_i^{\beta^*} \\ \cS\ne0}} c_{i,\cS} \sum_{\substack{\cS' \in \cS_{i'}^{\prime\beta^*} \\ \cS'\ne0}} c_{i',
        \cS'}\\
        &\leq \frac{d^2Y_{\max}^2}{np},
    \end{align*}
    where $\cM_i:= \{i':|\cN_i \cap \cN_{i'}|\geq1\}$.
\end{proof}

==> a5-related-works.tex <==
\section{Related Works} \label{app:related-work}
Besides risk mitigation and meeting logistical constraints, recent works have shown that rollout designs can be useful for causal inference under interference. \citet{han2022detecting} present statistical tests to detect the presence of interference using rollout designs. Our work differs from theirs in that our focus is estimating treatment effects under interference, not detecting its presence. \citet{ari2023rollout} leverage rollout designs as part of a model selection mechanism to select a ``best'' model for interference. While they also study the TTE, their focus is on its identification conditions and how rollout designs aid in satisfying them. \citet{viviano2020experimental} does not leverage rollout designs, instead considering a two-wave experiment that uses a pilot study in the first wave to minimize variance in causal effect estimation from a main experiment in the second wave. Unlike our two-stage approach, their two-wave design does not utilize a staggered rollout. Furthermore, \citet{viviano2020experimental} requires \textit{anonymous interference} \citep{hudgens2008toward, liu2014large, li2022random}, which posits that only the number, not identity, of treated units affects an individual's outcome, whereas our approach does not require this assumption. The approach most similar to our work is \cite{cortez2022neurips}, since they consider staggered rollout designs for estimating the TTE alongside the class of models and estimators we analyze in the present work. We present a modification to their experiment design that reduces the mean squared error (MSE) in many settings.
\cycomment{Questions about references. Do all assume anonymous interference?}

Many prior approaches in the literature on causal inference under interference consider cluster randomized designs \citep{sobel2006randomized,hudgens2008toward,liu2014large,auerbach2021local,ugander2013graph, gui2015network, eckles2017design, brennan2022cluster, ugander2023randomized}. These works focus on exploiting structural assumptions on the underlying interference network to reduce bias in the difference in means estimator or reduce variance in the Horvitz-Thompson estimator via cluster randomized designs. Some of these works rely on the assumption of \textit{partial interference}, which posits that the underlying network is made up of disjoint groups and interference only occurs within, not across, groups \citep{sobel2006randomized,hudgens2008toward, liu2014large, auerbach2021local, bhattacharya2020causal}. Other works are devoted to proposing cluster randomized designs that exploit knowledge about the network and its structure to minimize the number of edges that cross clusters in settings where partial interference may not hold \citep{ugander2013graph, gui2015network, eckles2017design, brennan2022cluster, ugander2023randomized}. 

Additional approaches to causal inference under interference focus on exploiting potential outcomes modeling assumptions in their methodology while considering simpler, unit-randomized designs instead of, or in addition to, cluster-randomized designs \citep{cai2015social, chin2019featureengineering, gui2015network, parker2017optimal, toulis2013estimation}. These approaches assume linear or generalized linear potential outcomes models, reducing the estimation task to regression. A drawback of these approaches is that they assume anonymous interference and that the individuals in the population share the same outcomes model.
To address this, \citet{cortez2022neurips} introduced a flexible class of potential outcomes models that allow for heterogeneous treatment effects by relaxing the anonymous interference assumption and instead imposing the $\beta$-\textit{order interactions} assumption, where interference effects are constrained to small subsets of the population, also explored in \cite{cortez2023jci, lowordercluster-2024}.
In both our work and \cite{cortez2022neurips}, the class of estimators under consideration are based on polynomial interpolation, where a key insight is that under a $\beta$-order potential outcomes model, the expected average outcome of the population is a $\beta$-degree polynomial in the treatment level. This style of estimator was first introduced by \citet{yu2022PNAS} for the case when the polynomial is degree $1$. \citet{cortez2022neurips} generalized this to polynomials of higher degree and established the connection to polynomial interpolation but did not use any clustering in their design. A drawback is that when the polynomial degree is greater than $1$, the estimator has prohibitively high variance, especially when the treatment probability is small. The present work addresses this with a two-stage experimental design to reduce variance in polynomial interpolation estimators for the TTE. A key contribution of \cite{yu2022PNAS} and \cite{cortez2022neurips} is the unbiased estimation of causal effects \textit{without any knowledge of the underlying interference network}, which the majority of prior approaches require. Our approach also does not require network knowledge.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
